FRB 20121102A: images of the bursts and the varying radio counterpart

As more Fast Radio Bursts (FRBs) are being localised, we are learning that some fraction have persistent radio sources (PRSs). Such a discovery motivates an improvement in our understanding of the nature of those counterparts, the relation to the bursts themselves and why only some FRBs have PRSs. We report on observations made of FRB 20121102A with the MeerKAT radio telescope. Across five epochs, we detect the PRS associated with FRB 20121102A. Our observations are split into a cluster of four epochs (MJD 58732 - 58764) and a separate single epoch about 1000days later. The measured flux density is constant across the first four observations but then decays by more than one-third in the final observation. Our observations on MJD 58736 coincided with the detections of 11 bursts from FRB 20121102A by the MeerTRAP backend, seven of which we detected in the image plane. We discuss the importance of image plane detections when considering the commensal transient searches being performed with MeerKAT and other radio facilities. We find that MeerKAT is so sensitive that within a two-second image, we can detect any FRB with a flux density above 2.4mJy at 1.3GHz and so could localise every FRB that has been detected by CHIME to date.

==> notes.tex <==

The average fluence of a CHIME detected FRB is 8$\pm$11\,Js\,ms. The average fluence of the FRB 121102 bursts detected by MeerKAT, \citep{2020MNRAS.496.4565C}, is 1$\pm$1\,Jy\,ms. Of the bursts reported in \citet{2020MNRAS.496.4565C}, the brightest two were detected in the image plane: bursts ten and eleven. These bursts had fluences of 0.4 and 4.13\,Js\,ms, respectively. There are bursts of fluence higher than 0.4\,Js\,ms, such as burst 7, but there is no image plane detection. The average noise in the burst 7 images is 8,7\,mJy compared to 1.6\,mJy in the burst 11 images. The noise in the burst 7 images is over 5 times higher. In addition to the noise varying across the length of the observations, the bursts were not detected across the whole observing band due in part to their spectral evolution but also due to varying noise levels across the band. The band was split into eight spectral windows and only in some of the bands were we able to detect the bursts. The variations in noise in different spectral windows for the same 2\,second integration may be partially due to different flagging levels in different parts of the band. For example, in the observations from MJD 58764, the 8 different spectral windows have flagging levels of \%. The different flagging percentages correspond different noise levels in the resulting images. Spectral windows zero, three and six have the highest levels of slagging and also have some of the highest noise levels. Therefore, moving forward one of the largest issues facing detections of FRBs is RFI mitigation. Large flagging fractions in certain parts of the observing band will prevent future image place detections because the flagging will drastically increase the noise in the resulting images. 


Therefore, even though some faint bursts are detectable, i.e. those $<$1\,mJy, those brighter than a few mJy are most likely to be detected. We also note that the rms noise in the final images could be lowered with regular phase calibrator observations combined with self-calibration. Given the detections that have been made in this data set, we can conclude that it is likely that we would be able to detect most of the CHIME FRBs in MeerKAT image plane data. 

Image plane detections of FRBs are incredibly important as they allow direct arcsecond-accuracy localisation as oppose following up repeating FRBs that were first detected by single dish telescopes. FRBs can be searched for commensally in all previous and future 2\,second integration data. 


A further limiting factor of image plane FRB detections is the dispersion measure. If the dispersion measure of the FRB is too high then the difference in the arrival time of the burst between the top and bottom of the band will be longer than the integration time (2\,s). For MeerKAT, with a central frequency of 1.26\,GHz and a bandwidth of 0.86\,GHz, the largest dispersion measure for an FRB before the pulse is smeared out across more than one integration is 560\,pc\,cm\textsuperscript{-3}. Of course, this assumes that the beginning of the pulse arrives at the beginning of any single integration. In reality, the limiting DM would be much lower as it depends on when exactly the burst begins to arrive. Arriving too late in an integration would mean we'd have to sum two integrations together, at this point the noise would wash out the signal. 


PWN

\begin{table*}
    \centering
    \begin{tabular}{ccccc}
    \hline
    Burst &  Frequency (GHz) & Peak Flux density (mJy/beam)  &  Integrated Flux density (mJy) & rms noise (mJy/beam)\\
    \hline
     3 & 1.5&$1.32\pm0.2$ & $1.6\pm0.4$ & 0.4\\
     5 & 1.5&$2.4\pm0.1$ & $0.90\pm0.4$ & 0.3 \\
     7 & 1.1 & $2.3\pm0.2$ & $1.4\pm0.4$ & 0.6 \\
     8 & 1.5&$1.8\pm0.1$ & $1.4\pm0.2$ & 0.3 \\
     9 & 1.5&$1.9\pm0.2$ & $1.8\pm0.4$ &  0.3\\
     10 & 1.5&$1.46\pm0.07$ & $1.3\pm0.2$ & 0.4\\
     11 & 1.5&$1.03\pm0.07$ & $1.07\pm0.19$ & 0.3\\
    \hline
    \end{tabular}
    \caption{A table of the integrated and peak flux densities of the bursts detected along side the rms noise value measured in the image of each detected burst.}
    \label{tab:bursts}
\end{table*}
